Your Classifier can Secretly Suffice Multi-Source Domain Adaptation

Multi-Source Domain Adaptation (MSDA) deals with the transfer of task knowledge from multiple labeled source domains to an unlabeled target domain, under a domain-shift. Existing methods aim to minimize this domain-shift using auxiliary distribution alignment objectives. In this work, we present a different perspective to MSDA wherein deep models are observed to implicitly align the domains under label supervision. Thus, we aim to utilize implicit alignment without additional training objectives to perform adaptation. To this end, we use pseudo-labeled target samples and enforce a classifier agreement on the pseudo-labels, a process called Self-supervised Implicit Alignment (SImpAl). We find that SImpAl readily works even under category-shift among the source domains. Further, we propose classifier agreement as a cue to determine the training convergence, resulting in a simple training algorithm. We provide a thorough evaluation of our approach on five benchmarks, along with detailed insights into each component of our approach.

==> tables/Office31_OfficeHome.tex <==
\newcommand{\CC}{\cellcolor{gray!14}{}}

\begin{table}[t]
	\center
	\begin{footnotesize}
	

\begin{tabular}{ cc }   % top level tables, with 2 columns
A. Office-31 & B. Office-Home \\  
	
	
	\adjustbox{valign=t}{
		\setlength\tabcolsep{2.0pt} 
		\begin{tabular}{c|c|ccc|c}
		  %  \Xhline{1.0pt}
			&Models
			&$\rightarrow$D
			&$\rightarrow$W 
			&$\rightarrow$A 
			&Avg  \\
			
% 			&&&&&\\
			
			\hline
			\multirow{6}{*}{\begin{turn}{90}\makecell{SB}\end{turn}} &ResNet&99.3&96.7&62.5&86.2\\
                &DDC&98.2&95.0&67.4&86.9\\
                &DAN&99.5&96.8&66.7&87.7\\
                &D-CORAL&99.7&98.0&65.3&87.7\\
                &RevGrad&99.1&96.9&68.2&88.1\\
                &RTN&99.4&96.8&66.2&87.5\\
			
			\hline
			\multirow{3}{*}{\begin{turn}{90}\makecell{SC}\end{turn}} &DAN&99.6&97.8&67.6&88.3\\
                &D-CORAL&99.3&98.0&67.1&88.1\\
                &RevGrad&99.7&98.1&67.6&88.5\\
			
			\hline	\multirow{4}{*}{\begin{turn}{90}\makecell{MS}\end{turn}}&DCTN&99.3&98.2&64.2&87.2\\
                    % &MFSAN$_d$&99.7&97.9&68.1&88.6\\
                    % &MFSAN$_m$&99.9&98.3&71.5&89.9\\
                    &MFSAN&99.5&98.5&72.7&90.2\\
                &\CC SImpAl$_{50}$&&&&\\
                &\CC SImpAl&&&&\\
        
		\end{tabular}} &
		
		\adjustbox{valign=t}{
		\setlength\tabcolsep{2.0pt} 
		\begin{tabular}{c|c|cccc|c}
		  %  \Xhline{1.0pt}
			&Methods
			&$\rightarrow$A
			&$\rightarrow$C
			&$\rightarrow$P
		    &$\rightarrow$R	
		    &Avg  \\
			
			
			
			\hline
			\multirow{5}{*}{\begin{turn}{90}SB \end{turn}}&ResNet&65.3&49.6&79.7&75.4&67.5\\
            &DDC&64.1&50.8&78.2&75.0&67.0\\
            &DAN&68.2&56.5&80.3&75.9&70.2\\
            &D-CORAL&67.0&53.6&80.3&76.3&69.3\\
            &RevGrad&67.9&55.9&80.4&75.8&70.0\\
			
			\hline
			\multirow{3}{*}{\begin{turn}{90}SC \end{turn}} &DAN&68.5&59.4&79.0&82.5&72.4\\
&D-CORAL&68.1&58.6&79.5&82.7&72.2\\
&RevGrad&68.4&59.1&79.5&82.7&72.4\\

			
			\hline	\multirow{5}{*}{\begin{turn}{90}MS \end{turn}} &MFSAN$_d$&69.8&60.2&80.2&81.0&72.8\\
&MFSAN$_m$&71.1&61.9&79.3&80.8&73.3\\
&MFSAN&72.1&62.0&80.3&81.8&74.1\\

&\CC SImpAl$_{50}$&&&&&\\
&\CC SImpAl&&&&&\\
        
		\end{tabular}}
		
		\end{tabular}
		
	\end{footnotesize}
\caption{\textbf{Results on Office-31 and Office-Home dataset}. `SB' stands for Single Best, `SC' stands for Source Combined. `MS' stands for Multi-source approaches. SImpAl$_{50}$ uses ResNet-50 as the backbone. }
\label{table:office31_officeHome}
 \vspace{-0.4cm}
\end{table}


==> tables/domainnet.tex <==



\newcommand{\BL}{\color{black!40!green}}
% \newcommand{\BU}[1]{\color{black!40!green}\textbf{#1}}
\newcommand{\BU}[1]{#1}


\newcommand{\BO}[1]{\textbf{#1}}
\newcommand{\BV}[1]{\color{black!10!blue}{\em #1}}

\newcommand{\redbold}[1]{{\textbf{#1}}}

\begin{table}
\centering
\small
{
\setlength\tabcolsep{3.5pt} 
\begin{tabular}{l|c |c |c| c| c |c | c |c}
% \Xhline{1.0pt}
% \multirow{2}{1.2cm}{ mm,up,sv,sy $\rightarrow$ mt}
&
Models & 
$\rightarrow$clp &  
$\rightarrow$inf  & 
$\rightarrow$pnt & 
$\rightarrow$qdr &    
 $\rightarrow$rel  & 
 $\rightarrow$skt  & 
\BU{Avg} \\ 
% &&&&&&&& \\

%  \Xhline{0.7pt} 
\hline
\multirow{6}{*}{\begin{turn}{90}SB\end{turn}} 
& Source Only & 39.6$\pm$0.5 & 8.2$\pm$0.7 & 33.9$\pm$0.6 & 11.8$\pm$0.6 & 41.6$\pm$0.8 & 23.1$\pm$0.7 & \BU{26.4}$\pm$0.7\\

 &DAN~\cite{lng15} &  39.1$\pm$0.5 & 11.4$\pm$0.8 & 33.3$\pm$0.6 & \redbold{16.2}$\pm$0.3& 42.1$\pm$0.7  & 29.7$\pm$0.9 & \BU{28.6}$\pm$0.6\\
 &RTN~\cite{RTN} &  35.3$\pm$0.7 & 10.7$\pm$0.6 & 31.7$\pm$0.8 & 13.1$\pm$0.6& 40.6$\pm$0.5  & 26.5$\pm$0.7 & \BU{26.3}$\pm$0.7\\
  &JAN~\cite{JAN} &  35.3$\pm$0.7 & 9.1$\pm$0.6 & 32.5$\pm$0.6 & 14.3$\pm$0.6& 43.1$\pm$0.7  & 25.7$\pm$0.6 & \BU{26.7}$\pm$0.6\\
%   &DANN~\cite{DANN} &  37.9$\pm$0.6 & 11.4$\pm$0.9 & 33.9$\pm$0.6 & 13.7$\pm$0.5& 41.5$\pm$0.6  & 28.6$\pm$0.6 & \BU{27.8}$\pm$0.6\\
    &ADDA~\cite{adda} &  39.5$\pm$0.8 & 14.5$\pm$0.6 & 29.1$\pm$0.7 & 14.9$\pm$0.5& 41.9$\pm$0.8  & 30.7$\pm$0.6 & \BU{28.4}$\pm$0.7\\
%  &SE~\cite{SE} & 31.7$\pm$0.7 &  12.9$\pm$0.5  & 19.9$\pm$0.7 & 7.7$\pm$0.4 &33.4$\pm$0.5&26.3$\pm$0.5&\BU{22.0}$\pm$0.6 \\ 
 &MCD~\cite{MCD} & 42.6$\pm$0.3 &  19.6$\pm$0.7  & 42.6$\pm$0.9 & 3.8$\pm$0.6 &50.5$\pm$0.4&33.8$\pm$0.8&\BU{32.2}$\pm$0.6 \\
                                 
                                     
 \Xhline{0.7pt} 
\multirow{6}{*}{\begin{turn}{90}SC\end{turn}} 
&Source Only & 47.6$\pm$0.5  & 13.0$\pm$0.4 & 38.1$\pm$0.4   & 13.3$\pm$0.3 & 51.9$\pm$0.8 & 33.7$\pm$0.5 & \BU{32.9}$\pm$0.5\\
&DAN~\cite{lng15}& 45.4$\pm$0.4&	12.8$\pm$0.8&	36.2$\pm$0.5&	15.3$\pm$0.3&	48.6$\pm$0.7&	34.0$\pm$0.5&	\BU{32.1}$\pm$0.5  \\
 &RTN~\cite{RTN} & 44.2$\pm$0.5&	12.6$\pm$0.7&	35.3$\pm$0.5&	14.6$\pm$0.7&	48.4$\pm$0.6&	31.7$\pm$0.7&	\BU{31.1}$\pm$0.6\\
&JAN~\cite{JAN}& 40.9$\pm$0.4&	11.1$\pm$0.6&	35.4$\pm$0.5&	12.1$\pm$0.6&	45.8$\pm$0.5&	32.3$\pm$0.6&	\BU{29.6}$\pm$0.5  \\
% &DANN~\cite{DANN}& 45.5$\pm$0.5&	13.1$\pm$0.7&	37.0$\pm$0.6&	13.2$\pm$0.7&	48.9$\pm$0.6&	31.8$\pm$0.6&	\BU{32.6}$\pm$0.6  \\
&ADDA~\cite{adda}& 47.5$\pm$0.7&	11.4$\pm$0.6&	36.7$\pm$0.5&	14.7$\pm$0.5&	49.1$\pm$0.8&	33.5$\pm$0.4&	\BU{32.2}$\pm$0.6  \\

% &SE~\cite{SE}& 24.7$\pm$0.3&	3.9$\pm$0.4&	12.7$\pm$0.3&	 7.1$\pm$0.4&	22.8$\pm$0.5&	9.1$\pm$0.4&	\BU{16.1}$\pm$0.4  \\

&MCD~\cite{MCD}& 54.3$\pm$0.6&	22.1$\pm$0.7&	45.7$\pm$0.6&	7.6$\pm$0.4&	58.4$\pm$0.6&	43.5$\pm$0.5&	\BU{38.5}$\pm$0.6  \\

\Xhline{0.7pt}
\multirow{4}{*}{\begin{turn}{90}MS\end{turn}} 
&DCTN~\cite{xu2018} &48.6$\pm$0.7  & 23.5$\pm$0.5  &48.8$\pm$0.6  &7.2$\pm$0.4& 53.5$\pm$0.5 & 47.3$\pm$0.4 & \BU{38.2}$\pm$0.5 \\

&M\textsuperscript{3}SDA & 57.0$\pm$0.7 & 22.1$\pm$0.6  &50.5$\pm$0.4  &4.4$\pm$ 0.2& 62.0$\pm$0.4 & 48.5$\pm$0.5 & \BU{40.8}$\pm$ 0.5\\

&M\textsuperscript{3}SDA&57.2$\pm$0.9  & 24.2$\pm$1.2 & 51.6$\pm$0.4 &5.2$\pm$0.4  & 61.6$\pm$0.8& \redbold{49.6}$\pm$0.5 &  \BU{41.5}$\pm$0.7\\

& M\textsuperscript{3}SDA-$\beta$ &\redbold{58.6}$\pm$0.5& \redbold{26.0}$\pm$ 0.8& \redbold{52.3}$\pm$0.5& 6.3$\pm$0.5& \redbold{62.7}$\pm$0.5& 49.5$\pm$0.7& \redbold{42.6}$\pm$0.6 \\

& \CC SImpAL$_a$ &&&&&& \\
& \CC SImpAL &&&&&& \\

\Xhline{0.7pt}
\multirow{3}{*}{\begin{turn}{90}OrR\end{turn}} 

&AlexNet &65.5$\pm$0.5  & 27.7$\pm$0.3  &57.6$\pm$0.4 &68.0$\pm$0.5& 72.8$\pm$0.6 & 56.3$\pm$0.5 & \BU{58.0}$\pm$0.5 \\

&ResNet101 &69.3$\pm$0.3  & 34.5$\pm$0.4  &66.3$\pm$0.6 &66.8$\pm$0.5& 80.1$\pm$0.5 & 60.7$\pm$0.4 & \BU{63.0}$\pm$0.5 \\

&ResNet152 &71.0$\pm$0.6  & 36.1$\pm$0.6  &68.1 $\pm$ 0.4  &69.1$\pm$0.5 & 81.3$\pm$0.4 & 65.2$\pm$0.5 & \BU{65.1}$\pm$0.5 
                                  
% \Xhline{1.0pt}
\end{tabular}
}
\vspace{0.1cm}
\caption{
\textbf{Multi-source domain adaptation results on the DomainNet dataset.} When the target domain is \textit{quickdraw}, the multi-source methods perform worse than single-source and source only baselines, which indicates negative transfer~\cite{pan2010survey} occurs in this case. ({\BV{clp}}: \textit{clipart}, {\BV{inf}}: \textit{infograph}, {\BV{pnt}}: \textit{painting}, {\BV{qdr}}: \textit{quickdraw}, {\BV{rel}}: \textit{real}, {\BV{skt}}: \textit{sketch}.)
}
\label{table_lsdac}
\vspace{-0.1cm}
\end{table}





%%%%%%%%%%%%%%





%%%%%%%%%%%%%%






%%%%%%%%%%%%%%%%%




% \begin{table}[htbp]
% 	\centering
% 	\footnotesize
% 	\caption{Accuracy (\%) on {DomainNet} for MSDA (ResNet-101).}
% 	\label{table:domainnet_sota}
% 	\begin{tabular}{lccccccc}
% 		\toprule
% 		Method  (:T)      &:c & :i & :p & :q & :r & :s & Avg  \\
% 		\midrule
% 		ResNet \cite{he2016Resnet} & 47.6          & 13.0          & 38.1          & 13.3          & 51.9          & 33.7          & 32.9 \\
% 		DAN~\cite{Long15DAN}         & 45.4          & 12.8          & 36.2          & 15.3          & 48.6          & 34.0          & 32.1 \\
% 		RTN~\cite{Long16RTN}         & 44.2          & 12.6          & 35.3          & 14.6          & 48.4          & 31.7          & 31.1 \\
% 		JAN~\cite{Long17JAN}  & 40.9 & 11.1 & 35.4 & 12.1 & 45.8 & 32.3 & 29.6\\
		
% 		ADDA~\cite{ADDA2017} & 47.5 & 11.4 & 36.7 & 14.7 & 49.1 & 33.5 & 32.2 \\
% 		SE~\cite{SE2018} & 24.7 & 3.9 & 12.7 & 7.1 & 22.8 & 9.1 & 16.1 \\
% 		MCD~\cite{MCD2018} & 54.3 & 22.1 & 45.7 & 7.6 & 58.4 & 43.5 & 38.5 \\
		
% 		\midrule
		
% 		DCTN~\cite{xu2018deep}        & 48.6          & 23.5          & 48.8          & 7.2           & 53.5          & 47.3          & 38.2 \\
% 		$\rm M^{3}SDA$~\cite{peng2018moment}       & 58.6          & 26.0          & 52.3          & 6.3           & 62.7          & 49.5          & 42.6 \\
% 		\textbf{MCC} \cite{XX}      & \textbf{63.0}          & \textbf{29.8}          &  \textbf{56.4}          &  \textbf{15.6}             &  \textbf{66.4}            &  \textbf{54.1}            &  \textbf{47.6}   \\
% 		\midrule
% 		\textbf{Ours}      & \\
	    
% 	    \bottomrule
		
% 	\end{tabular}
% \end{table}

==> tables/officeCaltechAndImageClef.tex <==
% \newcommand{\CC}{\cellcolor{gray!14}{}}

\begin{table}[t]
	\center
	\begin{footnotesize}
	

\begin{tabular}{ cc }   % top level tables, with 2 columns
A. Office-Caltech10 & B. ImageCLEF \\  
	
	
	\adjustbox{valign=t}{
	
	\setlength\tabcolsep{4.2pt} 
	
	\begin{tabular}{c|c|cccc|c}
		  %  \Xhline{1.0pt}
% 			\multirow{2}{*}{} 
			
			&Models
			&$\rightarrow$W
			&$\rightarrow$D
			&$\rightarrow$C
			&$\rightarrow$A
			&Avg
			\\ 
% 			&&&&&& \\
			\hline
			\multirow{2}{*}{\begin{turn}{90}\makecell{SC}\end{turn}}	&Source only& 99.0	& 98.3& 87.8	& 86.1	  &	92.8	\\
			&DAN		& 99.3	& 98.2 & 89.7	& {
			\textbf{94.8}}	  &	95.5	\\
			\hline				
			\multirow{10}{*}{\begin{turn}{90}\makecell{MS}\end{turn}}
			&Source only & 99.1  & 98.2 & 85.4 &88.7 & 92.9 \\				
			&DAN	&99.5	&	99.1	& 89.2	& 91.6 	& 94.8	\\
			&DCTN & 99.4 & 99.0 & 90.2 & 92.7 & 95.3\\
			&JAN	&99.4	&	\textbf{99.4}	& 91.2	& 91.8 	& 95.5\\
			&MEDA & 99.3 & 99.2 & 91.4 & 92.9 & 95.7 \\
			&MCD & 99.5 & 99.1 & 91.5 & 92.1 & 95.6 \\
			
			&M\textsuperscript{3}SDA	&99.4		&99.2	& 91.5	&94.1 &	96.1	\\
			&M\textsuperscript{3}SDA-$\beta$	&	\textbf{99.5}	& 99.2	&  \textbf{92.2}	& 	94.5	 & 	\textbf{96.4}	\\
% 			\Xhline{1.0pt}
        &\CC SImpAl$_a$&&&&&\\
        &\CC SImpAl&&&&&\\
		\end{tabular}} &
		
		\adjustbox{valign=t}{
		\setlength\tabcolsep{4.0pt} 
		\begin{tabular}{c|c|ccc|c}
		  %  \Xhline{1.0pt}
			
			&Models
			&$\rightarrow$P
			&$\rightarrow$C
			&$\rightarrow$I
			&Avg  \\
			
			\hline
			\multirow{6}{*}{\begin{turn}{90}\makecell{SB}\end{turn}} &ResNet&74.8&91.5&83.9&83.4\\
			&DDC&74.6&91.1&85.7&83.8\\
			&DAN&75.0&93.3&86.2&84.8\\
			&D-CORAL&76.9&93.6&88.5&86.3\\
			&RevGrad&75.0&96.2&87.0&86.1\\
			&RTN&75.6&95.3&86.9&85.9\\
			
			\hline
			\multirow{3}{*}{\begin{turn}{90}\makecell{SC}\end{turn}} &DAN&77.6&93.3&92.2&87.7\\
			&D-CORAL&77.1&93.6&91.7&87.5\\
			&RevGrad&77.9&93.7&91.8&87.8\\
			
			\hline	\multirow{4}{*}{\begin{turn}{90}\makecell{MS}\end{turn}}
			&DCTN&75.0&95.7&90.3&87.0\\
            &MFSAN&79.1&95.4&93.6&89.4\\
            
        &\CC SImpAl$_a$&&&&\\
        &\CC SImpAl&&&&\\
		\end{tabular}}
		
		\end{tabular}
		
	\end{footnotesize}
\caption{\textbf{Results on Office-Caltech10 dataset}. A,C,W and D represent \textit{Amazon}, \textit{Caltech}, \textit{Webcam} and \textit{DSLR}, respectively. All the experiments are based on ResNet-101 pre-trained on ImageNet.}
\label{table:office_caltech_imageclef}
 \vspace{-0.4cm}
\end{table}

